On the Reliability of Test Collections for Evaluating Systems of Different Types

As deep learning based models are increasingly being used for information retrieval (IR), a major challenge is to ensure the availability of test collections for measuring their quality. Test collections are generated based on pooling results of various retrieval systems, but until recently this did not include deep learning systems. This raises a major challenge for reusable evaluation: Since deep learning based models use external resources (e.g. word embeddings) and advanced representations as opposed to traditional methods that are mainly based on lexical similarity, they may return different types of relevant document that were not identified in the original pooling. If so, test collections constructed using traditional methods are likely to lead to biased and unfair evaluation results for deep learning (neural) systems. This paper uses simulated pooling to test the fairness and reusability of test collections, showing that pooling based on traditional systems only can lead to biased evaluation of deep learning systems.

==> 04-reusability.tex <==
\section{Reusability of test collections}
\label{sec:reusability}

==> 07-result_prev.tex <==
\section{Results and analysis}
\label{sec:result}

\begin{figure}
%\centering
\subfloat[Neural Systems \\ Traditional Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/ndcg10_neural_depth10traditional.png}
}
\subfloat[Traditional Systems\\ Neural Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/ndcg10_traditional_depth10neural.png}
}
\hspace{0mm}
\subfloat[Random Split 1 \\ Split 2 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/ndcg10_split1_depth10split2.png}
}
\subfloat[Random Split 2 \\ Split 1 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/ndcg10_split2_depth10split1.png}
}
\caption{NDCG@10 values for document retrieval task, where (a) neural runs are evaluated using pools generated from traditional runs, (b) traditional runs are evaluated using pools generated from neural runs, (c) runs from one random split (split 1) are evaluated using pools generated from the remaining split (split 2) of runs, and (d) runs from the remaining random split (split 2) are evaluated using pools generated from the remaining split (split 1) of runs.}
\end{figure}

\begin{figure}
%\centering
\subfloat[Neural Systems \\ Traditional Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/ndcg10_neural_depth10trad.png}
}
\subfloat[Traditional Systems\\ Neural Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/ndcg10_trad_depth10neural.png}
}
\hspace{0mm}
\subfloat[Random Split 1 \\ Split 2 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/ndcg10_split1_depth10split2.png}
}
\subfloat[Random Split 2 \\ Split 1 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/ndcg10_split2_depth10split1.png}
}
\caption{NDCG@10 values for passage retrieval task, where (a) neural runs are evaluated using pools generated from traditional runs, (b) traditional runs are evaluated using pools generated from neural runs, (c) runs from one random split (split 1) are evaluated using pools generated from the remaining split (split 2) of runs, and (d) runs from the remaining random split (split 2) are evaluated using pools generated from the remaining split (split 1) of runs.}
\end{figure}

\begin{figure}
%\centering
\subfloat[Neural vs. Traditional Systems \\ Traditional Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/mrr_neural_depth10traditional.png}
}
\subfloat[Neural vs. Traditional Systems\\ Neural Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/mrr_traditional_depth10neural.png}
}
\hspace{0mm}
\subfloat[Random Split 1 \\ Split 2 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/mrr_split1_depth10split2.png}
}
\subfloat[Random Split 2 \\ Split 1 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/mrr_split2_depth10split1.png}
}
\caption{MRR values for document retrieval task, where (a) neural runs are evaluated using pools generated from traditional runs, (b) traditional runs are evaluated using pools generated from neural runs, (c) runs from one random split (split 1) are evaluated using pools generated from the remaining split (split 2) of runs, and (d) runs from the remaining random split (split 2) are evaluated using pools generated from the remaining split (split 1) of runs.}
\end{figure}

\begin{figure}
%\centering
\subfloat[Neural Systems \\ Traditional Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/mrr_neural_depth10trad.png}
}
\subfloat[Traditional Systems\\ Neural Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/mrr_trad_depth10neural.png}
}
\hspace{0mm}
\subfloat[Random Split 1 \\ Split 2 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/mrr_split1_depth10split2.png}
}
\subfloat[Random Split 2 \\ Split 1 Depth-10 Pool]{
  \includegraphics[width=45mm]{plots/passageretrieval/mrr_split2_depth10split1.png}
}
\caption{MRR values for passage retrieval task, where (a) neural runs are evaluated using pools generated from traditional runs, (b) traditional runs are evaluated using pools generated from neural runs, (c) runs from one random split (split 1) are evaluated using pools generated from the remaining split (split 2) of runs, and (d) runs from the remaining random split (split 2) are evaluated using pools generated from the remaining split (split 1) of runs.}
\end{figure}

\begin{figure}
%\centering
\subfloat[Document retrieval task]{
  \includegraphics[width=0.5\linewidth]{plots/discovery-curve-docs.pdf}
}
\subfloat[Passage retrieval task]{
  \includegraphics[width=0.5\linewidth]{plots/discovery-curve-passages.pdf}
}
\caption{Cumulative count of relevant results at each rank cutoff. In document retrieval, neural runs find more relevant results at early cutoffs, but then are overtaken by traditional runs at later cutoffs. In passage retrieval, neural runs find more relevant results at all cutoffs.}
\end{figure}



==> 08-discussion.tex <==
\section{Discussion}
\label{sec:discussion}
